TGView3D System Description: 3-Dimensional Visualization of Theory Graphs

We describe TGView3D, an interactive 3D graph viewer optimized for exploring theory graphs. To exploit the three spatial dimensions, it extends a force-directed layout with a hierarchical component. Because of the limitations of regular displays, the system also supports the use of a head-mounted display and utilizes several virtual realty interaction concepts.

==> lib/kbibs/src/html/generate-html <==
#!/bin/bash

# Check that we have the right number of parameters, otherwise die. 
if [ "$#" -ne 3 ]; then 
  >&2 echo "Illegal number of parameters (expected 3, got $#). ";
  >&2 echo "Usage: $0 \$SRC \$DIST \$KWARC";
  >&2 echo "Generates html from .html and .xml files"; 
  exit 1;
fi

# read variables
SRC="$1"
DIST="$2"
KWARC="$3"

echo "Generating html from $SRC into $DIST"

# files
BIB_XSL="${SRC}html/bibliography.xsl"
BIB_ALL_XSL="${SRC}html/bibliography-all.xsl"


LTOPT="--quiet --bibliography=${DIST}ltxml/kcr.bib.xml --format=xhtml --path=${SRC}ltxml --preload=${SRC}ltxml/kwarcbibs.sty.ltxml"

## now we extract all the HTML from kcr.bib
TYPES='article incollection conference workshop thesis report unpublished misc wproceedings cproceedings cbook'
for i in $KWARC; do
    for j in $TYPES; do
	echo "Generating special LaTeX file ${DIST}tex/$i-$j.tex";
    	xsltproc --stringparam file $i-$j -o ${DIST}tex/$i-$j.tex ${BIB_XSL} ${DIST}ltxml/kcr.bib.xml;
	echo "converting it to XML";
	latexmlc ${LTOPT} --destination=${DIST}html/$i-$j.html ${DIST}tex/$i-$j.tex 2> >(tee ${DIST}tex/$i-$j.ltxlog >&2);
    done;
done;

for j in $TYPES; do
  echo "Generating special LaTeX file ${DIST}tex/$j.tex";
  xsltproc --stringparam type $j -o ${DIST}tex/$j.tex ${BIB_ALL_XSL} ${DIST}ltxml/kcr.bib.xml;
  echo "converting it to XML";
	latexmlc ${LTOPT} --destination=${DIST}html/$j.html ${DIST}tex/$j.tex 2> >(tee ${DIST}tex/$j.ltxlog >&2);
done;


==> lib/kbibs/src/kwarcnocites.tex <==
% kwarc citations, generated from kwarcpubs.bib with emacs M-x occur (and some manual
% work) update this from time to time. 
\mypubkeys{%
%2014
cjucovschi:interaction_integration:14,
HKR:flexary:14,
Koh:SearchInterfacesMath:2014,
Rabe:literal:14,
KalRab:hollight:14,
IanJucKoh:sdsal2oc14,
IanJucKoh:sps14,
Kohlhase:dmesmgm14,
DumGinKoh:katsd14,
IanJucKoh:sdm14,
CarFarKoh:rsckmt14,
KohIan:crsmmd14,
Kohlhase:mkmtobbtg14,
%2013
KohMihSperTes:mfs13,
LanAspCar:CICMWiP13,
KohlhaseEtAl:FullSemanticTransparency:2013,
KohManRab:aumftg13,
KohKoh:ssl13,
RabKoh:WSMSML13,
DoeKohLin:oamim13,
IanKohRabUrb:tmmliotaa13,
DoeKoh:mamim13,
Kohlhase:tffm13,
Kohlhase:kmsedcs13,
%2012
DML12,
Rabe:ttbor12,
Koh:NavigationInMathDocs2012,
 JucEth12:redsys,
cdavid:mscthesis,
KohDavGin:fspmco12,
ProKoh:mwssofse12,
DavJucKoh:safusa12,
HorKohRab:emfsl12,
Kohlhase:ppte12,
KohIan:ssmk12,
LIDBSKA:MSC-SKOS12,
Kohlhase:mdadmls12,
LanKoh:MathMashups12,
KohRab:som12,
LangeEtAl:MSC-LOD12,
MSC-SKOS,
HR:tptp:12,
dumbrava:msc,
horozal:msc,
alecu:bsc,
ignatov:bsc,
iacob:msc,
IR:ui:12,
CHMR:compiling:12,
RS:vertrans:12,
CHIR:casl:12,
HR:patterns:12,
Iancu:mcdl12,
IanRab:mocdl12,
% 2011
HenZho:tlxx11:biblatex,
DFRU:cicm:11,
DFRU:cicmwip:11,
GNRS:lfmtpmlpa:11,
CGL:PublishingUnitsQuantitiesPost11,
CGL:PublishingUnitsQuantities11,
zamdzhiev:bsc:math,
SEPUBLICA11,
Lange:KrextorSystem11,
DC:BauDenkMalNetz11,
OCAS2011,
MathWiki11,
KohJuc:pcmpm11,
IanKohRab:tmmlof11,
ProKoh:mwsofse11,
KohDavGin:psewads11,
LKDGKMMZ:PlanetaryExecutableSTEM11,
KohKoh:micvl11,
KohKoh:tfndc11,
KohKoh:vl11,
CodHorKoh:palai11,
HorIacJuc:cscpnrr11,
GinStaKoh:latexmldaemon11,
DavGin+:fmspscdl11,
AutDav+:wfcs11,
% 2010
KohKohLan:difcsmse10:biblatex,
KohRabSac:fvip11,
KohRabZho:tmlmrsca10:biblatex,
JucKoh:sidesc10:biblatex,
KohKohLan:ssffld10:biblatex,
DKLRZ:PubMathLectNotLinkedData10,
StaKoh:tlcspx10,
StaGinDav:calxmec10,
GinJucAnc:alsaacl09,
GriWolKoh:tcbdme09,
StaGinDav:maacl09,
StaGinDav:acsmlcl09,
KohLemSchSch:fmccp09a,
ZhoKoh:tvsx09,
ZhoKoh:sdxvdt10,
Kohlhase:OMDoc1.6spec,
Kohlhase:OMDoc1.3,
Kohlhase:OMDoc1.6book,
Kohlhase:OMDoc1.6primer,
Kohlhase:OMDoc1.6processing,
Kohlhase:OMDoc1.6projects,
TLCSK:SemanticBugSearch09,
DavKoh:umoattsea09,
DavKoh:umoattsfp09,
DavKoh:qio09,
RabKoh:abrsom09,
KGLZ:JOBADabstract09,
DKLRZ:JOBAD-MMT-AIMashup10,
GLR:WebSvcActMathDoc09,
LK:MathOntoAuthDoc09,
LK:MathOntoAuthDoc09:FGWM,
calMue:fprcu09,
TR:CM:FPRCAU,
OpenMathWiki:on,
KohLemSchSch:fmccp09,
KohKoh:ccbss09,
KohKoh:sifemp09,
KohKoh:ccbssmt09,
Kohlhase:BootstrappingPragmaticStrictOMDoc,
RabeKohlhase:ExchangeModularKnowledge,
CM:CoPSW,
CM:CoPSW:DC,
TR:KLMMR:NfAD,
NM:CMoSSD,
TR:MK:CAAACoMN,
MK:CAAACoMN,
LBGBH08:SIOC-argumentation,
HuKeKo:gcccp94,
Kohlhase:SemanticInteractionDesignDiss:biblatex,
TR:MK:CoPiMeL,
JG:CRAiMDuOaS,
KohPro:MWSmanual,
LangeGonzalez:SWiM-Sentido08,
Lange:Krextor09,
Zholudev:TNTBaseVDs10,
Zholudev:TNTBaseRESTful,
Zholudev:TNTBaseRESTful:web,
Rabe:MMT,
krextor:on,
LangeEtAl:ArgumentationSWiM08,
KohKoh:csbs08,
LangeEtAl:ArgumentationSWiMSCooP08,
MK:CTACoPT,
Kohlhase:wcl08,
KohMelSie:oma99,
Kohlhase:ar03,
CM:TCwIO,
CM:TACCMCOP,
MueKoh:cpme08,
MueKoh:cptsma08,
NRM08:fst,
KohKoh:AssessmentInSACHS,
KohKoh:SACHSCoverage10,
KohKoh:stuas09,
KohKoh:mteuas09,
Ionita:ExtractingRDFFromOMDoc08,
URL:omdocspec,
VZ:resprop,
AI:internrep,
lange:swim-demo08,
cm:mn:08,
KLMMR:AoNiLMD,
lange:swim-notation-semantics08,
Lange:SWiM-OpenMath08,
LangeMcLRabe:FlyspeckWiki08,
KMR:NoLMD08,
StaKoh:tax08,
KohAncJuc:MWS08:biblatex,
Lange:SWiMSciColl07,
CarlisleEd:MathML10,
NRM:DA05,
MK:Proofs:omdoc2vf06,
MK:ProofObjects:omdoc2vf06,
NRM:resprop,
NRM:wp1:07,
panta:on,
janta:URL,
pr-project:on,
Panta:web,
pr-project:web,
Panta:demo,
Panta:gencs,
AA:BTIPR08,
Panta:cs:precourse:on,
SWiM:on,
URL:sTeX:head,
sTeX-mode:on,
URL:sTeX-slides:head,
NRM:lwa06,
MW:lwa07,
NRM:kij07,
KuKeKo:bo96,
mueller07:lectora-resprop,
Lange07:kwepsy,
Lange07:swimplus-resprop,
wikipedia:omdoc,
Panta:CSFall2007,
LanKoh:swmkm07,
Lange:swmkm-tr07,
Pesikan:cwcr06,
Misev:sumo2omdoc,
HorKohRab:tal10,
HKR:sequences:11,
AR:lamkrip:11,
HR:folsound:10,
CHKMRS:lfhets:11,
IKR:mizar:11,
rabeEA:isabelle-lf:10,
RI:isabelle:10,
rabe:combining:10:biblatex,
CHKMR:hiding:11,
CHKMR:hiding:10,
IR:foundations:10,
DLR:jobad:10,
kristina:ml_fol,
rabe:isalf:10,
CHKMRS:lfhets:10,
DHS:algebra:09,
rabeEA:folsound-lf:09,
project:mmtlf,
RS:twelfmod:09,
AR:lamkrip:09,
AR:lamkrip_long:09,
KLMMR:notations-tr:2009,
rabeEA:presentation:09,
rabe:gi:09,
HR:folsound:09,
project:latin,
rabe:mmt:09,
RK:keappa:08,
SR:dfol_fol:08,
BRS:tptphol:08,
rabe:thesis:08,
RPSS:moloss:07,
GMPRS:catlog:07,
rabe:graphs:07,
rabe:instlf:07,
rabe:moloss:06,
rabe:dfol:06,
rabeEA:promela:05,
cmueller:thesis:10,
BenBroKoh:csil06,
BenBroKoh:lmcs09,
Kohlhase:oaifocdi00,
KohFra:rkcimss01,
sTeX:online,
LATIN:online,
JOMDoc:on,
PhysML:web,
OMBase:web,
locutor:on,
OMDocDocOnto:on,
KWARC:web,
JOBAD:demo,
JOBAD:on,
docOnto:web,
Kohlhase:GenCSI:on,
Kohlhase:GenCSIproblems:on,
Kohlhase:GenCSIsolutions:on,
Kohlhase:GenCSII:on,
Kohlhase:PlanetGenCS:on,
Kohlhase:GenCSIIproblems:on,
Kohlhase:GenCSIIsolutions:on,
KohSuc:asemf06,
ArmKoh:cpmsbko00,
arXMLiv-buildsys:online,
arXMLiv-frontend:online,
arXMLiv:online,
arXMLiv:demo:online,
sTeXIDE:online,
AspKoht:mimp02,
NorKoh:efnrsmk07,
KohKoh:rmvp07,
KohKoh:skmfe08,
BenzmuellerEtAl:otama97,
BenKoh:ehor98,
BlaBos:atpfnlu98,
ClaKoh:ratp03,
ClaKoh:sda03,
HuKe:katfad94,
HKK94a,
HuKe94b,
AK:mbase06,
LanKoh:swim06,
Kohlhase:albwo06,
Kohlhase:shlssc06,
NRM:omdoc2vf06,
Kohlhase:OAFFlexiForms10,
Kohlhase:SemiformalizationDef09,
OAFF:online,
JoKo:uiaelc94,
KeKo:mpwri97,
KeKoSo:icawpp96,
KohKoh:cdad04,
JesKohSei:DMV04,
KohKoh:copmem06,
HilKohSta:copmem06,
KohKoh:esmk05,
Kohlhase:hoatp98,
Kohlhase:atpm98,
Kohlhase94b,
Kohlhase:uiostt92,
KohAng:tccmvc03,
HanKoh:atcnl03,
KohKol:ttmlu00,
KohSut:amcas02,
Kohlhase:autxdm03,
LanKoh:swmkm06,
SiekmannEtAl:pdwo02,
TNTVDSkel:URL,
TNTVDUseCases:URL,
TNTBaseIntegration,
Rabe:TNTBaseMMTPlugin,
OMDoc:svn,
OMDocRNC:URL,
OMDocXSD:URL,
mathweb.org:svn,
OMDocXSL:URL,
OMDoc-mailinglists:URL,
mkm-mailinglists:URL,
ek:dsxcc,
Kohlhase:hoatp-lnai,
MuKo:pr07-small,
KohSim:escpmge01,
CD:inference-rules,
OMDocDTD:URL,
FormalSafeProposal,
MWSProj:on,
SieHes:adgui98,
CPoint:Web,
AspKohSac:dtdop03,
Laubner:utgmm07,
w3c:web:mathml,
W3C:MathML2:biblatex,
CarIon:MathML03,
AutEbe:dkmvc03,
BenBroKoh:hose04,
BenBroKoh:cexf08,
FraKoh:mrmkrdb99,
BenKoh:lahotp98,
BenKoh:mefhol97,
BenKoh:rfhm97,
BenKohBro:hose03,
BlaKoh:ics04,
BlaBos:iacs98,
BlaBosKoh:iacs01,
BlaBos:iacs99,
BusCapCar:2oms04,
EggGarKoh:sid98,
KerKoh:fmds94,
KerKoh:pwtc96,
EggKoh:dcqs97,
EggKoh:uqs97,
FraKoh:cwmik99,
FraKoh:dm99,
FraHes:aoidms99,
FraKoh:mabdl99,
FraKoh:sdmaomkb00,
GarKoh:cpid97,
GarKoh:fahou96,
GarKoh:hocuanls96,
GarKohKon:hocuala99,
GarKohKon:hocuala97,
GarKohKon:chou96,
GarKoh:hounls96,
GarKoh:hfhou96,
GarKohLeu:cahou96,
BanKoh:mmlof07,
HeJuKoSo:aidms98,
HuangEtAl:SR-92-20,
HuKe:oapde94,
HuKe:oapde92,
HuKe94a,
HutKoh:msihocu00,
HutKoh:acvotlc97,
KohSch:homvr95,
HuaKerKoh:oma95,
Kohlhase:msholbrp94,
HuKo:acvotl95,
JoKo93,
KeKo94,
KeKo:arcfp96,
KerberKohlhase97a,
KeKo:atcfpf96,
KeKo93a,
KeKoSo:icaipp98,
KeKoSo96,
Kohlhase:ophcie05,
Kohlhase:omdoc05,
Kohlhase:emPowerPoint,
Kohlhase:MediaOrMedeaSociety,
Kohlhase:CPointMUI,
Kohlhase:CPointWiederverwendbarerContent,
Kohlhase:UserAsPrisoner,
Kohlhase:horwc93,
Kohlhase92,
Kohlhase:mgfdrt00,
Kohlhase:OMDoc1.2,
AKo:SPoKMaEL,
BosKoh:icos-editorial03,
MuKo:pr07,
KoMaMu:MViDCaNS,
WaMu:TCoPSfIMA,
CM:TtIaSosCoP07,
CM:PoEIaSSCoPbosmosdawt,
Lange:swmkm-ui07,
KohMueMue:dfncimk07,
KohLanRab:pmcfe07,
Kohlhase04:stex,
Kohlhase:omfmd01,
Kohlhase:corfl00,
Kohlhase:otisadt00,
Kohlhase:otormd00,
Kohlhase:sat96,
Kohlhase:hotwc96,
Kohlhase:hot95,
Kohlhase94a,
Kohlhase:amosho94,
Kohlhase:hoosr94,
Kohlhase:aupfeh93,
Kohlhase91,
Kohlhase89,
Kohlhase:ulsmf08,
KohCar:ggm03,
KohDev:bvm03,
DevKoh:stm03,
KohKol:ramgpm03,
KohKon:mgfdrt99,
KohKon:hoatpnls98,
KohKus:clausdlc97,
KohKus:dlc97,
KohKusPin:attsfl96,
KoPf:uialcw93,
KerKoh:rwb11,
WolGriKoh:udc11,
KohSch99:homvr,
KohSim:inid02,
PinKoh:flfdt00,
Giceva:WSActiveMathDoc09,
Broecheler:tmsw07,
LOUI98-UITP,
SieHes:loui99,
SieBen:acgap00,
SieKohMel:oema98,
ZimKoh:tmsbdmr02,
planetmathredux:on,
pantarheiredux:on,
MathWebSearch:online,
Kohlhase:pplp:ctan,
Kohlhase:pdrp:ctan,
Kohlhase:pfepr:ctan,
Kohlhase:ed:ctan,
KohAmb:smmssl:ctan,
Kohlhase:ipsmsl:ctan,
Kohlhase:smp:ctan,
Kohlhase:reqdoc:ctan,
Kohlhase:physml:ctan,
Kohlhase:dcm:ctan,
Kohlhase:workaddress:ctan,
Kohlhase:assignment:ctan,
Kohlhase:problem:ctan,
Kohlhase:sref:ctan,
Kohlhase:metakeys:ctan,
Kohlhase:rdfmeta:ctan,
Kohlhase:owl2onto:ctan,
Kohlhase:smms:ctan,
Kohlhase:tbscml:ctan,
Kohlhase:clbscm:ctan,
Kohlhase:smomdl:ctan,
Kohlhase:smmtf:ctan,
Kohlhase:ssmtl:ctan,
Kohlhase:atpm98chapter,
Kohlhase:codemlspec,
brownhorozal07,
Kohlhase:friomkb01,
LZ:OWLChangeRefactorXMLDB10,
DLKA:ProtoBrowserListedBuildSMW10,
HutKoh:OMoCProposal06,
KohMue:added-value07,
GraZho:rest2011,
Zholudev:TNTBaseRESTful:base,
Zholudev:TNTBaseORES:base,
krextor:webpage,
Lange:PhD:plain,
Lange:PhD:book:plain,
OpenMathWiki:base,
RDFaHostLanguages,
Lange:SWiMSubversionClient,
Lange:wiki-argu-draft,
flyspeck-wiki:web,
swim-bugzilla,
swim-roadmap,
NMueller:PhD,
Kohlhase:InvasiverEditor,
Kohlhase:pufmp08,
Planetary:on,
PlanetaryEPCMilestone:on,
EPCsystem:on,
LinkedLectures,
PlanetGenCS:on,
PlanetLATIN:on,
PlanetBox:on,
Kohlhase:SemanticPowerPoint,
Kohlhase:PPTforChildren,
Kohlhase:EngagingPPT,
Kohlhase:LearnerAndLearningTechnology,
Reichel:FolksonomiesAsEmbodiedActions,
Reichel:EmbodiedConceptualizations,
KohlhaseReichel:FuzzyLinePrivatePublic,
Anca:NLMPforATS09,
Anca:matesearch07,
Horozal07,
DHK:algebra:09,
IVEB:SemEnabBusProcDisc10,
DGKC:eMath30,
FA:MathKnowReprEduSemWebLearnStyle10,
DR:filtering:10,
Dumbrava:sshelf,
rabe:bslreview:10,
KohKoh:tcmff10,
ako:MicrodataVsRDFa,
Kohlhase:MailGenericMetadata2008,
Kohlhase:STS-RelaxNG08,
KohSuc:mwssse07,
xslt:web,
mmlkit:web,
vzamdzhiev:bscthesis,
mcirlanaru:bscthesis,
OntoIOpOASIS2001,
Stamerjohanns:latexmleditor,
AA:IPRaaCT,
OMDoc:wiki,
OMDocUG:web,
Grigore-10,
latexml:branch:online,
latexml-daemon,
Ginev:OnDigitalCorpora,
Ginev:TowardsABuildSystemForDigitalCorpora,
MGG:email,
Kuryla:OWLtoOMDocTranslation09,
Ontohub,
lange05:wiki,
lange06:wikiblog,
% from crossrefs
OpenJEM07,
JEM08,
IJCAI03-KR,
CADE15-WS-PSMAD,
ICOS00,
BosKoh:ICOS2-LJIGPL04,
ICOS01,
KI06,
CADE15-WS-AI,
CALCULEMUS00,
MKM05
}
%%% Local Variables: 
%%% mode: LaTeX
%%% TeX-master: "kwarcpubs"
%%% End: 

